NumGLUE: A Suite of Fundamental yet Challenging Mathematical Reasoning Tasks

Given the ubiquitous nature of numbers in text, reasoning with numbers to perform simple calculations is an important skill of AI systems. While many datasets and models have been developed to this end, state-of-the-art AI systems are brittle; failing to perform the underlying mathematical reasoning when they appear in a slightly different scenario. Drawing inspiration from GLUE that was proposed in the context of natural language understanding, we propose NumGLUE, a multi-task benchmark that evaluates the performance of AI systems on eight different tasks, that at their core require simple arithmetic understanding. We show that this benchmark is far from being solved with neural models including state-of-the-art large-scale language models performing significantly worse than humans (lower by 46.4%). Further, NumGLUE promotes sharing knowledge across tasks, especially those with limited training data as evidenced by the superior performance (average gain of 3.4% on each task) when a model is jointly trained on all the tasks as opposed to task-specific modeling. Finally, we hope that NumGLUE will encourage systems that perform robust and general arithmetic reasoning within language, a first step towards being able to perform more complex mathematical reasoning.

==> sections/notes.tex <==
\sm{
\paragraph{Key points:}
\begin{itemize}
    \item We talk about datasets like MATH, mathematics etc. but we really do not need that complicated math in NLP, specialized systems like Mathematica, MATLAB are still good at that, what we need is basic arithmetic operations +-/* , not even equations. These needs to be embedded with various intricacies of NLP which involve various tasks such as QA, NLI, RC etc. and various reasoning skills involving some sort of common or very simple domain knowledge.
    \item MATH is hard, to our surprise we show that fundamental tasks are also harder for GPT3, and so those - the foundation blocks- need to be solved before pouncing on hard problems like MATH etc.
    \item We have a map that shows how this is the simplest hierarchy of benchmarks requiring minimum operations.
    \item We experiment with GPT3 and show that decomposition based method helps model improve its performance, but it is far from being solved.
\end{itemize}}


Neural language models powered by datadriven approaches have achieved human level performance across several NLP tasks. However, we still require machines that understand the world well enough to perform reasoning. This capability would give rise to new opportunities for real-world applications such as education, medicine, and scientific discovery \cite{clark2016my} \cite{clark2015elementary}. Additionally, numbers help us to reason in everyday tasks ranging from buying vegetables to reading newspaper to understanding economic situation, survey results, sports, climate change, and election. Since numbers make our conversation accurate, the skill to reason with them is of primary importance in understanding natural language. \cite{dehaene2011number,ravichander2019equate,frank2008number}.
% {It is debatable whether type 2 question is more less complex than estimation and adversarial category. Clarify that complexity here refers to the number and complexity of mathematical operation. In our case, these are 1-step and fairly straightforward problems}

\sm{Copied from positive reviewer comments that will help frame our story better: 
\begin{itemize}
    \item "This paper takes the next, and important, step in the slow but steady evolution of numerical reasoning in a natural language (typically, QA) setting. Several past datasets have been collected, standardized, and compiled into various forms for different numerical tasks. The innovation here is NUMBERGAME, to prompt systems to convert various forms of numerical description/questions into a single standardized format to support generic numerical reasoning."
    \item "Overall this is very nice work, very timely, and helps advance NL-based engines in the important area of being able to convert text into and reason inside ‘number space’. The paper is clear, logical, and includes various interesting facets of analysis about the numbers, types, and other aspects of the data in Sections 5 and 7 (too often, dataset papers do not include this sort of description!)."
    \item "The benchmark is designed to combine different formats (e.g. both question answerign and NLI) as well as different domains (e.g. scientific knowledge and commonsense). The paper presents a number of baseline results using existing systems as well as an existing numerical reasoning system that has been trained to also predict the sub-task that each question belongs to. There is also a novel information retrieval augmented model."
    \item "Reasoning about numbers and measures is essential to communication, and it can occur in drastically different contexts. Current benchmarks focus on specific sub-problems and are often amenable to short-cuts. The field could benefit from more robust and complete benchmarks."
    \item "1.) A  lot  of  work  has  recently  tried  to  solve numerical reasoning and execution abilities which makes need for a consistent evaluation benchmark for numerical reasoning quite important.)  The authors have used a nice way to convert different numerical reasoning tasks into a common RC style format.)  They have also proposed three automatically generated datasets and constructed a knowledge base  of  formulas  that  can  be  useful for the community"
    \item "Just like Glue and ORB, it might be nice to have many datasets related to numerical reasoning provided in a single format that allows to evaluate models for numerical reasoning over multiple datasets."
    \item "Reasoning about numbers and measures is  essential  to  communication,  and  it  can  occur in drastically different contexts.   Current benchmarks focus on specific sub-problems and are often amenable to short-cuts.   The field could benefit from more robust and complete benchmarks."
\end{itemize}
}


% Neural Language models have achieved near-human performance in several Natural Language Understanding benchmarks (NLU). However, numerical reasoning remains to be one of the skills, these models struggle at. We humans deal with numbers in our everyday tasks ranging from reading economics news in the morning to watching sports scores in the night. In the pursuit of building AI systems that possess human-level understanding, it is important to impart the capability to reason over numbers in these models. 

% Several datasets have been proposed to foster research in numerical reasoning in natural language questions answering context. Examples include ....
% 
Even though Neural language models such as GPT \cite{radford2018improving}, BERT \cite{devlin2018bert} and RoBERTa (\cite{liu2019roberta} have become standard tools across several language understanding tasks, they can not perform complex forms of reasoning, specifically numerical reasoning \cite{wallace2019nlp}. 
Several datasets have been proposed to foster research in numerical reasoning in natural language understanding and QA context. Examples include DROP \cite{dua2019drop}, EQUATE \cite{ravichander2019equate}, MathQA \cite{amini2019mathqa} and the Mathematics dataset \cite{saxton2019analysing}. But each of these focuses on a specific format. For example, DROP is in RC setting. EQUATE and MathQA are in NLI and QA setting respectively. Several neuro-symbolic models have been proposed in response to the numerical reasoning  datasets. Examples include NumNet+v2 \cite{ran2019numnet}, BERT Calculator \cite{andor2019giving} and tag-based multi-span extraction model \cite{efrat2019tag}. These models have achieved high performance on their corresponding test sets but struggled to solve questions of a different format or a different dataset. For example, Pre-training BERT Calculator on CoQA \cite{reddy2019coqa} followed by fine-tuning on DROP leads to improved results on DROP, however the performance on CoQA drops drastically \cite{andor2019giving}. Humans can understand numerical reasoning questions irrespective of their format and answer appropriately. But, format conversion is a challenge in NLP. Many recent efforts to exploit multiple datasets remain largely restricted to a single format. The challenge is further evidenced by the underperformance of several recent approaches to build a common model for various NLP
tasks using Google T5 \cite{khashabi2020unifiedqa, raffel2019exploring}. Format conversion is even more challenging for numerical reasoning, as there have been large performance drops across two datasets in slightly different formats such as DROP and CoQA using BERT-Calculator.

\begin{table*}[!htb]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Type}                                                                          & \textbf{Original question}                                                                                                                                                                                                                                                       & \textbf{Transformation}                                                                                                                                                                                                                                                                                & \textbf{Knowledge required}                                          & \textbf{Answer} \\ \hline
\begin{tabular}[c]{@{}l@{}}Numerical \\ commonsense \\ knowledge required\end{tabular} & \begin{tabular}[c]{@{}l@{}}A man can lift one box in each\\ of his hands. How many boxes can\\ a group of 5 people hold in total?\end{tabular}                                                                                                                                   & Not applicable                                                                                                                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}A human being has \\ 2 hands\end{tabular} & 10              \\ \hline
\begin{tabular}[c]{@{}l@{}}Domain knowledge \\ required\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}How many units of $H_2$ are required\\ to react with 2 units of  $C_2H_4$ to\\ form 2 units of  $C_2H_6$?\end{tabular}                                                                                                                                & Not applicable                                                                                                                                                                                                                                                                                         & $H_2 + C_2H_4 = C_2H_6$                                              & 2               \\ \hline
\begin{tabular}[c]{@{}l@{}}Qualitative \\ Commonsense \\ knowledge \\ required\end{tabular}           & \begin{tabular}[c]{@{}l@{}}A person wants to get shopping\\ done  quickly. They know that \\ they can get through the checkout \\ at big store faster than they can at\\  small store.  The store they go to\\  finish quickly is?\\  (A) big store (B) small store\end{tabular} & \begin{tabular}[c]{@{}l@{}}A person wants to get shopping \\ done quickly. They know that\\ they can get through the check-\\ out at big store in 5 minutes \\ whereas it can take 20 minutes at\\ small store. The store they go\\ to finish quickly is? (A) big store\\ (B) small store\end{tabular} & Not applicable                                                       & big store       \\ \hline
Completion format                                                                      & \begin{tabular}[c]{@{}l@{}}Joan found 70 seashells on the\\  beach. She gave Sam some of \\  her seashells.  She has 27 seashell\\  left. How many seashells did she\\  give to Sam?\end{tabular}                                                                                & \begin{tabular}[c]{@{}l@{}}Joan found 70 seashells on the \\ beach. She gave Sam some of\\ her seashells.She has 27 seas-\\ hells left. She gave \_\_\_\_\_ \\seashells to Sam?\end{tabular}                                                                           & Not applicable                                                       & 43              \\ \hline
\end{tabular}
}
\caption{Samples from the NUMBERGAME benchmark}
\label{tab:sample1}
\end{table*}


Since numerical reasoning is generic and independent of any particular format, there exists  a strong need for a benchmark which can evaluate abilities of models in performing question format independent numerical reasoning. Additionally, for numerical reasoning technology to have the best possible application, it must be able to process language and reason in a way that is not exclusive to a single format, task, dataset or domain. In pursuit of this goal, we introduce NUMBERGAME, a multifaceted dataset that builds upon existing datasets where we add some new types. Such a compilation by including datasets with limited training data is intended to encourage the development of general models that can address diverse question formats. For building a more practical numerical reasoning system, NUMBERGAME demands four additional capabilities  beyond numerical reasoning (i) figuring out the question format directly from data (ii) finding a way to train the system incorporating a wide variety of question types (iii) incorporating commonsense knowledge (iv)  handling data imbalance across formats.
%On the other hand, humans with sound understanding of numbers can perform multiple types of numerical reasoning. One may wonder whether the same can be done by a single language model. 
% However, these datasets are constrained to solve one kind of numerical reasoning at a time. E.g. DROP dataset expects the system to resolve references in a question accompanied by a passage and perform discrete operations
% over them (such as addition, counting, or sorting). Similarly, EQUATE dataset expects the system to do quantitative reasoning in a textual entailment setting. On the other hand, Humans with sound understanding of numbers can perform multiple types of numerical reasoning. One may wonder whether the same can be done by machines. Figure \ref{comparison} illustrates this. In order to evaluate the actual performance of machines in understanding  numbers, we incorporate 9 different kinds of question types while creating the proposed dataset. To the best of our knowledge, our work is the first one that proposes a dataset to simultaneously do numerical reasoning of various types. 
% As a first step towards this goal, we have considered basic numerical reasoning i.e. addition, subtraction, multiplication and division and their applications in different contexts.

% Additionally, our benchmark can help models leverage the benefits of multi-task learning where models can decide when to do transfer learning from one task to other \cite{McCann2018decaNLP}. This concept makes more sense in case of numbers for two reasons. First, numerical knowledge and understanding is a generic concept and doesn't differ across tasks. Second, we have relatively smaller datasets in maths, so zero shot or few shot learning will largely accelerate our research in quantitative reasoning. 

% Neural NLP models like GPT \cite{radford2018improving}, BERT \cite{devlin2018bert} and RoBERTa (\cite{liu2019roberta} are now the standard tool across language understanding, even solving basic reading comprehension and NLI datasets. Despite this, these models can not perform complex forms of reasoning, specifically numerical reasoning \cite{wallace2019nlp}. Recently, several neuro-symbolic models like NumNet+ \cite{ran2019numnet}, BERT Calculator \cite{andor2019giving} and tag based multispan extraction model \cite{efrat2019tag} have been proposed to perform numerical reasoning. All these models handle numbers using a symbolic engine. Even though they have performed well on DROP dataset, yet they are limited in terms of the type of questions and numerical operations they handle. We propose a generalized model based on combination of NumNet+ and tag based multispan extraction model which can answer any type of question. Additionally, to the best of our knowledge, our model is the first model which provides scope to incorporate common math knowledge. This is inspired from the observation that cheatsheet makes the task easier for humans while solving math questions of various types. Also, recent research showing the effect of knowledge in improving the performance of language models \cite{yang2018hotpotqa} \cite{mitra2019exploring} motivates further to add this feature in numerical reasoning.\\

% We compile a multifaceted dataset that builds upon existing datasets where we add some new types. Such a compilation is necessary and important to encourage the development of general models that can address all these types. 

%Additionally, our dataset can serve as a benchmark for multi-task learning in the numerical QA setting \cite{McCann2018decaNLP}. This concept makes more sense in case of numbers for two reasons. First, numerical knowledge and understanding is a generic concept and doesn't differ across tasks. Second, we have relatively smaller datasets in maths, so zero shot or few shot learning will largely accelerate our research in quantitative reasoning. To the best of our knowledge, our work is the first one that proposes a dataset and a task to simultaneously do numerical reasoning of various types. 


It is now well understood that natural language understanding requires knowledge beyond that is present in the specific text one is trying to understand. This was emphasized when the Winograd schema challenge was proposed \cite{levesque2012winograd} and Marcus \& Davis further emphasize this in their recent book \cite{marcus2019rebooting}. Indeed, several QA datasets have recently been proposed where answering requires reasoning with external knowledge of various kinds such as domain knowledge and commonsense knowledge \cite{bisk2019piqa,marino2019ok}. In our compilation, we add a significant number of QA pairs where external knowledge is needed to answer questions in numerical reasoning setting.
% Two of the new types we add are about questions that require external numerical knowledge, commonsense knowledge and domain knowledge. 
% While recently many QA datasets involving external knowledge have been proposed, ours incorporates them in a numerical reasoning setting. 




% However, these datasets are constrained to solve one kind of numerical reasoning at a time. But each of them are limited in their focus. 

% There are many datasets and many models. But each of them are limited in their focus. We compile a multifacted dataset that  builds up on existing datasets and we add some new types. Such a compilation is necessary and important to encourage development of general models that can address all these types. ... multi-task learning

%2 It is now well understood that natutal language understanding requires knowledge beyond that is present in the specific text one is trying to understand. This was emphasized when the Winograd challenge was proposed and Marcus \& Davis emphasize this in their recent book. Indeed, several QA datasets have recently been proposed where answering requires reasoning with external knowledge of various kinds such as domain knowledge and commonsense knowledge. In our compilation we add a significant number of QA pairs where external knowledge is needed to answer the numerical reasoning questions.

% Recently, several neuro-symbolic models like NumNet+ \cite{ran2019numnet}, BERT Calculator \cite{andor2019giving} and tag based multispan extraction model \cite{efrat2019tag} have been proposed to perform numerical reasoning. All these models handle numbers using a symbolic engine. Even though they have performed well on DROP dataset, yet they are limited in terms of the type of questions and numerical operations they handle. We propose a generalized model based on combination of NumNet+ and tag based multispan extraction model which can answer any type of question. Additionally, to the best of our knowledge, our model is the first model which provides scope to incorporate common math knowledge. This is inspired from the observation that cheatsheet makes the task easier for humans while solving math questions of various types. Also, recent research showing the effect of knowledge in improving the performance of language models \cite{yang2018hotpotqa} \cite{mitra2019exploring} motivates further to add this feature in numerical reasoning.\\
% Recently, several neuro-symbolic models have been proposed in response to the numerical reasoning  datasets. Examples include NumNet+v2 \cite{ran2019numnet}, BERT Calculator \cite{andor2019giving} and tag-based multi-span extraction model \cite{efrat2019tag}. Though they have performed well on the DROP dataset, they are limited in terms of the type of questions and numerical operations they handle. Also, they are overfitted to a specific dataset. For example, Pre-training BERT Calculator on CoQA \cite{reddy2019coqa} followed by fine-tuning on DROP leads to improved results on DROP, however the performance on CoQA drops drastically \cite{andor2019giving}. NUMBERGAME discourages overfitting and asks models to generalize.

% Pre-training on CoQA then fine-tuning on
% DROP lead to our best results on DROP, reported
% in Table 3. After fine-tuning on DROP, the model
% forgot how to do CoQA, with an overall F1 score
% of 52.2 on the CoQA dev set


We extend NumNet+v2 \cite{ran2019numnet}, the best one among the existing models for which code is publicly available. We add a question type\footnote{We will henceforth use format and type interchangeably} converter module on top of NumNet+v2 and create an initial baseline for our dataset. Noting that this model does not take into account external knowledge, we create a new enhanced architecture that does IR \cite{khot2019s, banerjee2019careful} with respect to a knowledge base we create, Mathkb to identify the needed knowledge. This is inspired by the observation that formula book and mathematical knowledge make the task easier for humans while solving math questions of various types. We then use this knowledge in the NumNet+V2 setting. This leads to an improved baseline. 
%hunting (searching for the missing knowledge)
% Contributions
% 1. Compilation
% 2. Knowledge
% 3. Improved Baseline

% Our contribution in this paper is as follows (i) We compile a multifaceted dataset involving eight different types and define a task to solve this in multi-task setting. In the process, we add four new types of data (ii) We introduce questions that require external numerical knowledge, commonsense knowledge and domain knowledge in the QA setting.
% (iii) We create a baseline by extending the NumNet+v2 model to handle questions of various types together (iv) We develop a new model that uses knowledge extraction using a formula sheet together with NumNet+V2; this leads to an improved baseline.

% \begin{itemize}
%     \item We compile a multifaceted dataset involving eight different types and define a task to solve this in multi-task setting. In the process, we add four new types of data.
%     \item We introduce questions that require external numerical knowledge, commonsense knowledge and domain knowledge in the QA setting.
%     \item We create a baseline by extending the NumNet+v2 model to handle questions of various types together.
%     \item We develop a model that uses knowledge hunting using a cheat sheet together with NumNet+V2; this leads to an improved baseline.
% \end{itemize}


% In recent years, there has been huge developments using datadriven AI applications. However, we still require machines that understand the world enough to perform reasoning. This capability would give rise to new opportunities for real-world applications like education, medicine, and scientific discovery \cite{clark2016my} \cite{clark2015elementary}. Numbers help us to reason in everyday tasks ranging from buying vegetables to reading newspaper to understanding economic situation, survey results, sports, climate change, election and medicine. Since numbers make our conversation accurate, the skill to reason with them is of primary importance in understanding natural language. \cite{dehaene2011number} \cite{ravichander2019equate} \cite{frank2008number}.
% \begin{figure}[h]
% \centering
% \includegraphics[width=9cm, height=8cm]{partialModel_New.png}
% \caption{Conventional models can not solve all types of questions vs our model which can}
% \label{comparison}
% \end{figure}

% Several datasets have been proposed to foster research in numerical reasoning such as DROP \cite{dua2019drop}, EQUATE \cite{ravichander2019equate}, MathQA \cite{amini2019mathqa} and the Mathematics dataset \cite{saxton2019analysing}. However, these datasets are constrained to solve one kind of numerical reasoning at a time. E.g. DROP dataset expects the system to resolve references in a question accompanied by a passage and perform discrete operations
% over them (such as addition, counting, or sorting). Similarly, EQUATE dataset expects the system to do quantitative reasoning in a textual entailment setting. On the other hand, Humans with sound understanding of numbers can perform multiple types of numerical reasoning. One may wonder whether the same can be done by machines. Figure \ref{comparison} illustrates this. In order to evaluate the actual performance of machines in understanding  numbers, we incorporate 9 different kinds of question types while creating the proposed dataset. To the best of our knowledge, our work is the first one that proposes a dataset to simultaneously do numerical reasoning of various types. As a first step towards this goal, we have considered basic numerical reasoning i.e. addition, subtraction, multiplication and division and their applications in different contexts.

% Additionally, our benchmark can help models leverage the benefits of multi-task learning where models can decide when to do transfer learning from one task to other \cite{McCann2018decaNLP}. This concept makes more sense in case of numbers for two reasons. First, numerical knowledge and understanding is a generic concept and doesn't differ across tasks. Second, we have relatively smaller datasets in maths, so zero shot or few shot learning will largely accelerate our research in quantitative reasoning. 

% Neural NLP models like GPT \cite{radford2018improving}, BERT \cite{devlin2018bert} and RoBERTa (\cite{liu2019roberta} are now the standard tool across language understanding, even solving basic reading comprehension and NLI datasets. Despite this, these models can not perform complex forms of reasoning, specifically numerical reasoning \cite{wallace2019nlp}. Recently, several neuro-symbolic models like NumNet+ \cite{ran2019numnet}, BERT Calculator \cite{andor2019giving} and tag based multispan extraction model \cite{efrat2019tag} have been proposed to perform numerical reasoning. All these models handle numbers using a symbolic engine. Even though they have performed well on DROP dataset, yet they are limited in terms of the type of questions and numerical operations they handle. We propose a generalized model based on combination of NumNet+ and tag based multispan extraction model which can answer any type of question. Additionally, to the best of our knowledge, our model is the first model which provides scope to incorporate common math knowledge. This is inspired from the observation that cheatsheet makes the task easier for humans while solving math questions of various types. Also, recent research showing the effect of knowledge in improving the performance of language models \cite{yang2018hotpotqa} \cite{mitra2019exploring} motivates further to add this feature in numerical reasoning.\\
% Our contribution in this paper is as follows:
% \begin{itemize}
%     \item In order to see whether a single system can answer any type of question involving numerical reasoning, we develop a benchmark dataset that incorporates nine different types of questions. 
%     \item We created five new types of numerical reasoning questions. Also, we cleaned and processed four types of question from existing datasets.  
%     \item We propose a generalized novel model which can answer any type of questions.
%     \item We introduce the concept of cheatsheet in numerical reasoning by providing scope to incorporate common math knowledge in our model.
% \end{itemize}

